Zero-Cost, Arrow-Enabled Data Interface for Apache Spark

Distributed data processing ecosystems are widespread and their components are highly specialized, such that efficient interoperability is urgent. Recently, Apache Arrow was chosen by the community to serve as a format mediator, providing efficient in-memory data representation. Arrow enables efficient data movement between data processing and storage engines, significantly improving interoperability and overall performance. In this work, we design a new zero-cost data interoperability layer between Apache Spark and Arrow-based data sources through the Arrow Dataset API. Our novel data interface helps separate the computation (Spark) and data (Arrow) layers. This enables practitioners to seamlessly use Spark to access data from all Arrow Dataset API-enabled data sources and frameworks. To benefit our community, we open-source our work and show that consuming data through Apache Arrow is zero-cost: our novel data interface is either on-par or more performant than native Spark.

==> reviews/hotstorage/a.tex <==
Review #13A
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Familiarity with one or more of this paper's topics

Novelty
-------
2. Incremental improvement

Writing quality
---------------
1. Needs improvement

Paper summary
-------------
This paper presents Arrow-Spark, a data connector framework to convert data between row-based Spark in-memory data processing with columnar data stores on disk.

Comments for author
-------------------
The paper is attacking an important problem and has constructed a solution that looks general and practical.

One major problem with the paper is that its research contributions are not well defined. Aside from the large amount of engineering work, it's not clear what research questions are answered. Design choices are given in an "as-is" manner, with little discussion on alternatives. As a result, the paper at times reads like a development document.

The batch size tuning discussion is interesting and has the potential to grow into deeper research exploration. The way it is currently presented, however, lacks clarity or consistency. For example, is the execution time per batch or total? Where does the large variance with Spark come from? If memory consumption is a big problem with Spark, why does it seem to work well with the largest batch size (2^15)? The text mentions that fitting the batch into L2 cache appears to give optimal results, while this does not seem to be supported by Fig 2? The conclusion given following the short discussion seems rather overly general and hasty.

Evaluation seems narrow, with very limited dataset configuration. The performance advantage over the Spark baseline is moderate in most cases.

Finally, it is not explained why the proposed scheme is labeled "zero-cost".

Suggestions for future work
---------------------------
I would encourage the authors to continue this research, focusing on answering new questions and making solid observations. Problems like batch size auto-tuning are interesting and require much more in-depth investigation and measurement, with varied data formats, sizes, and processing tasks.


==> reviews/hotstorage/b.tex <==
Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Familiarity with one or more of this paper's topics

Novelty
-------
2. Incremental improvement

Writing quality
---------------
2. Adequate

Paper summary
-------------
This paper builds a data connector layer that enables Spark to load data from many sources via a common dataset API. This enables one to separate computation from data access. Results show that this new connector offers similar performance to Spark's native data access methods, and in some cases, it offers improvements over the native method.

Comments for author
-------------------
Thanks for submitting to HotStorage 21. I appreciated your practical contributions. Below are some of my thoughts:

Strengths:

+ The idea has been implemented in a widely used system.
+ The new connector offers similar or better performance than Spark's native data access.

Areas for improvement:

- My major concern with this paper is that the ideas described, while useful, are narrow. There is little new in terms of ideas or results. For example, it is well known that batch sizes when reading and writing to storage must be carefully tuned to achieve good performance. As a result, I feel there is little for the larger community to learn some new things from this paper.

- The numbers reported may not reflect the actual speedup in real settings because there could be significant compute time in real workloads (that reduce the benefits brought about by a more efficient data-access method). If I am not wrong, the workloads the authors use do no or little actual computation.

Suggestions for future work
---------------------------
This paper is describing a useful data-access library that the current Spark ecosystem is missing. However, to make this work/paper more appealing to a broader set of storage/systems researchers and practitioners, I think it is important to separate the fundamental contributions from the implementation.

To this end, one fine point that the paper is bringing out is the possibility of lazy data materialization that the connector enables compared to other alternatives (e.g., PySpark + PyArrow). Is this is a fundamental problem with alternatives? If so, can you show that they cannot essentially load datasets bigger than the RAM available on the machine?

Another point would be to explore if the limitations of the native data-access methods are fundamental or not. For example, native Spark seems to be performing very poorly on the CSV dataset. Is this a fundamental limitation or just an implementation problem? How hard is it to fix if this is an implementation problem?


==> reviews/hotstorage/c.tex <==
Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
2. Familiarity with one or more of this paper's topics

Novelty
-------
2. Incremental improvement

Writing quality
---------------
2. Adequate

Paper summary
-------------
The topic of this paper is the efficient interoperability between distributed data processing ecosystems. In this work, a new zero-cost data interoperability layer between Apache Spark and Arrow-based data sources is designed, enabling practitioners to use Spark more efficiently. The interface is based on the Arrow Dataset API.

Apache Spark is a pervasive distributed data processing framework. Connecting Spark to other systems entails building connectors and converting data, which is a costly operation. In this case, using a universal interoperability layer instead enables more efficient data processing. Therefore, the novel interface proposes a new connector between Spark and the data layer to reduce I/O workload.

The article introduces the design and implementation of the Arrow-Spark framework，which provides an efficient interface between Apache-Spark and all Arrow-enabled data sources and formats. The data transmission starts with a read request coming from Spark. Then the interface uses Arrow C++ Dataset API to read data from Arrow datasets. At the same time, FileFormat will be selected according to the type of data to be read. After that, the interface uses the generated FileFormat to read/write data in batches. In the Arrow C++ Dataset API, a native Dataset instance is created, and each data batch is placed in memory as an Arrow IPC message, which is a columnar data format. Each Arrow IPC message is converted to an array of Spark-readable column vectors during the data conversion process. This operation cannot be avoided but is inefficient. In addition, for each new data type to support and for each new system to integrate with, new adapters or readers are required. Therefore, a universal connector is useful.

Experiments show that Arrow-Spark has scalability similar to Spark. Its advantage over Spark is the highest with 1-2 TB datasets. Furthermore, the Arrow-Spark presents very good acceleration effects in some data sets, especially in text-based file formats.

Overall, Arrow-Spark retains the original framework's performance and significantly improves it in some cases.

Comments for author
-------------------
The article’s idea is simple and has an excellent performance on some datasets. The design and architecture of the whole system are straightforward and easy to understand. However,  it is unclear the main contribution of this paper. You mentioned two major problems, but I did not see how you solve them. It would help if you highlighted your contribution.

The experiment chapter mentioned that the experiment of each configuration was run 31 times, and the first experiment value is discarded. Can you explain that such a cold start is uncommon in practical applications? If not, the first experimental value is also valuable experimental data and should not be discarded.

As mentioned in Experiment 4, the experimental results will be vastly different from the results shown in actual situations. So in actual applications, will it show the same trend as in the experiment, or whether the arrow-spark has such a performance in actual applications.
The sentence mentioned in Experiment 5 is not very clear: ”Although Spark is seemingly faster and higher selectivities, this is relative: on real-world datasets, even 1% selectivity could leverage datasets of over 1TB, at which point Arrow-Spark’s performance is superior.”

Except for Experiment 3, there is nothing that can reflect the advantages of the framework. You need to add experiments and explanations.

==> reviews/hotstorage/d.tex <==
Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
2. Familiarity with one or more of this paper's topics

Novelty
-------
2. Incremental improvement

Writing quality
---------------
3. Well-written

Paper summary
-------------
The paper describes the implementation of a connector between Spark and the Arrow Dataset API to provide Spark with in-memory access to data in row-based format for processing.  The proposal is to use this connector to provide an interface to all Arrow-enabled datasources, as an alternative to existing methods of providing datasource specific Spark connectors or using pySpark to retrieve data from pyArrow and perform the conversion.

Results comparing the existing Spark logic with that of the connector to read parquet and csv formats show the use of the connector is either on par or significantly improves performance.

Comments for author
-------------------
The paper is well-written and includes a thorough evaluation along with clear presentation and analysis of results.

Some positive design points:

+ Use of Arrow’s zero-copy streaming and IPC support to minimize the copy overhead

+ No additional development to provide Spark with access to other data sources already supported by the Arrow Dataset API

+ Advancements in Arrow to support new data formats or optimize processing will be immediately realized by Spark.

Suggestions for future work
---------------------------
Method for optimizing the small batch size processing overhead.

==> reviews/hotstorage/e.tex <==
Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
2. Familiarity with one or more of this paper's topics

Novelty
-------
2. Incremental improvement

Writing quality
---------------
2. Adequate

Paper summary
-------------
This paper proposes Apache-Arrow, a novel zero-cost data interoperability layer between Apache Spark and Arrow-based data sources through the Arrow Dataset API. The layer adopts a Java Native Interface (JNI) bridge implementation to enable communication between JVM-based Spark and C++-based Arrow Dataset API. The framework is evaluated with 5 separate experiments, and each experiment draws appropriate conclusions and provides advice for practitioners.

Comments for author
-------------------
The paper is generally easy to understand, but there are some obvious grammar and spelling mistakes. For example, the first sentence in the abstract, "their components highly specialized", lacks being verb "are"; in the first two paragraphs on the third page, the upper and lower case letters of "Core Arrow" and "Core Spark" are inconsistent.
Figure 1 is well drawn, but the contribution components in the figure are not explained in details.
Besides, the description of the JNI Bridge takes up half of the design section, so the work seems like an incremental extension for Arrow to support communication with Apache.
The experiments are carried out in a variety of ways, but the analysis of the experimental results is not comprehensive enough, which may be due to the limitation of space.
Some entries in the bibliography are incomplete, specifically, in references [3-4], [9-10], [12-14], [17], [23], [27], and [33], which are shown as "[n.d.]".

Suggestions for future work
---------------------------
The paper can be improved by providing more details on the contribution components in the design part as well as the analysis of the experimental results.
Spelling and grammar need to be checked throughout.

Comment @A1 by Reviewer D
---------------------------------------------------------------------------
During the PC discussion the two most significant concerns raised were the narrow scope of the paper, and the results provided.   While the solution proposed in the paper is a practical one the research contribution was unclear.   The individual reviews identify where improvements can be made to the data collection and analysis.


==> reviews/systor21/a.tex <==
Reviewer A

Thank you for submitting your work to SYSYOR. I think enabling Arrow support for any Spark API (not just pySpark) is a useful contribution and I like that your work will be open source. I also liked the JNI-based approach to improve the performance of any Arrow-related operations. Overall, the paper is well written and it was easy to follow.

1. My main issue was though that there does seem to be a Java implementation of Arrow (https://arrow.apache.org/docs/java/) and, looking at its feature set, it seems quite complete (https://arrow.apache.org/docs/status.html). Your claim that "there does not exist an Arrow Dataset implementation written in any JVM language" added to my confusion. You should clearly state, how you relate to this implementation and why you think it is insufficient. If it is because of missing features (e.g., the site above says that currently, Java only supports reading Avro), then my question would be, why is your approach better than implementing the missing features in Java or just making those available through JNI (not the entire Arrow API). If it is because of performance, then you should show that in your evaluation, by comparing to a Java-only implementation. I do think that your approach could be faster by using the core C++ implementation but you need to demonstrate that in the paper. Without a good reason why your more complex solution should be preferred over a simpler, Java only solution and why you can't use the existing Java Arrow implementation, the paper is incomplete.
S: Fixed. Hopefully made clear now


2. My second concern was the evaluation. While the existing experiments already cover several important use cases, I thought it was not enough to really provide a good idea of how native Spark compares to Arrow-Spark in different situations.

The SELECT query is very simplistic as it just scans the entire dataset. It would be good to experiment with different type of selections and vary the attributes, which are selected, and the selectivity. The current experiments only provide a single data point for performance, i.e., for a full table scan.

The dataset was also synthetic and, if I understood correctly, you only had a single 17GB file on your RAMDisk, which was then repeatedly read by Spark as different hard links. While this is ok for microbenchmarks to demonstrate any bottlenecks in the framework, I think it is important to also show numbers for actual data on disk. Otherwise, the results feel tailored towards just this single case and don't convey how Arrow and native Spark compare under more realistic settings, i.e. when input data is not read from memory.
S: Cannot fix with limited pages. Maybe say something along the lines 'due to space limitations, we cannot show...'?

3. Finally, as you said, pySpark already has support for Arrow. While you mention that this is very inefficient, it would be good to demonstrate this through experiments. I agree that some users might not want to use python just to get Arrow support but seeing the actual performance difference compared to your approach would make a strong argument that, even if users are already using python or are considering it for Arrow, the performance difference is prohibitive. In general, it is important to quantify, how inefficient pySpark really is.
S: I agree. Need to test if possible.



Other Comments:

1. Can you provide some more details of how exactly data is read from Arrow into an RDD/Dataframe in Spark? Does it require a copy?
S: Ehm what? We have Figure 1, black circlets 5 and 6 for that, with appropriate explanations.

2. Can you explain, how you minimized the overhead that JNI incurs? In general, it would be good to describe in a bit more detail, what the main novelties of your design are and what the difficulties were when implementing it in order to strengthen your contribution.
S: Sure, I can talk endlessly about the vile memory tricks I pulled, and the fact that Arrow greatly helps us with JNI. There is not much space however, and the space we have must first be used for other things. TODO: Come back here when almost done.

3. Are you supporting writes in your solution? How would writes need to be handled? I would be interested in also seeing comparisons of Spark and Arrow-Spark for the write path.
S: No writes! Only reads. We use parquet after all, so if you would even want to write, it would be writing new parquet files always, as parquet is not editable. TODO: Very maybe write about this.


4. In E1 and E2, what was the actual file format you used? You mention it was columnar data. Did you use Parquet for those experiments?
S: Changed: Explicitly stated we use parquet here indeed.

5. In Figure 3, it looks more like Spark and Arrow-Spark are converging rather than Arrow-Spark is getting better compared to Spark. Is this the actual trend? Maybe you can add another data point to confirm data and, if true, adapt the corresponding text.
S: Maybe, but not for this publication. It would take me 6 hours only to get the data. TODO: Extremely maybe, if pySpark is done.

6. I found the related work a bit weak. You say that there are also [8] and [31] but your implementation handles memory allocation differently, has better backwards compatibility, and supports more data types. These don't seem to be fundamental differences to the existing approaches though. What are the fundamental differences? Does your approach perform better? This part should be strengthened.
S: About [8]: The intel folks have no experiments, no paper. About [31] 'Spark: Cluster computing with workingsets': I do not know the difference. Probably: They have no universal data interface, which is kind of the main point about our approach.

Nits:

page 4: "[...] (left vertical axis) as well AS the relative speedup (right vertical axis)."
S: Fixed

page 5: "[...] parquet files in practical situations produceS vastly different [...]"
S: Fixed

Reviewer expertise
------------------
2. I have read some papers in this area

Would the community find this useful if published?
--------------------------------------------------
2. Yes

Correctness
-----------
2. Fixable flaws

Writing
-------
A. Easy to understand

Overall merit
-------------
C. Weak paper, though I will not fight strongly against it


==> reviews/systor21/b.tex <==
Reviewer B
Paper summary
-------------
The authors implement an extension of Spark data layer that allows to transparently support data sources providing Apache Arrow API in Spark. The implementation is quite straightforward with the main challenge, seemingly, being the fact that Spark is implemented in Scala while Apache Arrow in C++. The authors further perform extensive evaluation of the implementation, varying batch sizes, dataset sizes, data formats etc. Several lessons learned for practicioners are highlighted.

Comments for author
-------------------
Thank you for submitting your paper to SYSTOR'21! The paper's value, in my view, is that:

�� It solves very practical and specific issue; the code is open-sourced and, therefore, useful to practitioners
�� The impact of this implementation could be broad given the popularity of Spark and Apache Arrow
�� Extensive evaluation provides practitioners solid ideas on how to efficiently use the proposed code (that said, I have one big concern about evaluation, see below).

The paper is generally well structured and written (barring one comment below about Section 2).

At the same time, there are few significant weaknesses of the paper:

�� The effort, though practically useful, is mostly technical.  The paper has relatively low scientific impact.
S: Cannot do anything with this unhelpful stuff. This is systems research, not the dusty theoretical side of CS. 

��  In the Evaluation the authors state: "With local disk reading, the bottleneck lies in disk speed, and we cannot uncover any framework inefficiencies. To mitigate this issue, we decided to deploy data as close as possible to the CPUs." To me this sounds like performance is not an issue in real systems (that use persistent storage)! And yet the paper focuses on performance evaluation in a setup that never materializes in reality. (That said, the implementation itself is still useful because it allows new functionality - access to Arrow-based datasets).
S: This person doesn't get it: Using Arrow, we get access to any data type supported by Arrow, so Spark can stop it's endless fabrication of new connectors. 
S: Also, this person thinks the 'performance <of normal Spark?> is not an issue in real system'. Maybe we need to reprhase this quoted part. @Alex?

�� The authors state that currently one can use PySpark to access Arrow-based data sources in Spark. And the disadvantage of this approach is low performance. Unfortunately, no numbers are given to justify this statement and demonstrate how much faster is the  proposed new implementation.
S: I agree. Need to test if possible.

Other comments:

1. Paper structure: it was sudden to me to start reading about JVM and C++ in the beginning of Section 2. I'd like the authors to have a gentler introduction to why these details are relevant. The authors have some justification later in Section 2 - "Arrow-Spark JNI Bridge" and the following paragraph. I believe these paragraphs should go first and be expanded to clearly explain the challenge BEFORE the design description.
S: Yes, this might be a good idea. However, first stating what we have, and then why we have it, seems more sensible to me than first explaining why we have things, and later stating what the things are. I added a comment with a bit of 'why' before the first image reference circlet.


2. Would it make sense to implement Arrow in some JVM language rather than use JNI bridge? Is the only stopper on this path the amount of efforts required?
S: Yes, the implementation effort would be other-worldly. Besides, core Spark is much faster than any pure JVM implementation will ever be.

3. In many places the authors state that they run more experiments but could not include the results in the paper due to the length constrains. I encourage the authors to publish those results as a technical report and link it from the paper.
S: Is this a good idea @Alex?

4. It seems like the workloads in the given setup are mostly CPU/memory intensive. Would it be possible to include some information on CPU utilization for default Spark and Spark-Arrow?
S: Possible yes, but very painful. It would require a setup where we regularly monitor CPU usage of all nodes and add them together, much like Jayjeet and his Grafana plots. We either would need to write our own thing for that (much work) or use docker with Grafana (bloated, much work, will not work on DAS, where we performed experiments).


Reviewer expertise
------------------
2. I have read some papers in this area

Would the community find this useful if published?
--------------------------------------------------
2. Yes

Correctness
-----------
2. Fixable flaws

Writing
-------
A. Easy to understand

Overall merit
-------------
B. OK paper, but I will not champion it

==> reviews/systor21/c.tex <==
Reviewer C

Paper summary
-------------
The paper describes the implementation of a JNI based connector that enables Spark to access data served in various formats via the Apache Arrow API. The paper shows that Spark with their connector (Arrow-Spark) has comparable performance with default Spark.

Comments for author
-------------------
1. I would have liked the paper to make a stronger justification for the Spark connector for Arrow. For example, what does the connector enable that Spark doesn't provide natively? In particular, what formats are used by applications using Arrow, other than parquet and text files, and why are they beneficial?
S: This person really wants a list showing what formats/frameworks Arrow can access that Spark cannot. They do not understand that the whole point is that Arrow can take over the entire data adapter ecosystem from Spark, also being future proof, as more and more formats and frameworks support Arrow.
Need to make this more clear?

2. I think the paper needs to be more clear on the claims made in the paper. The introduction led to me to believe that Arrow-Spark would have significantly better performance than Spark. Based on your evaluation, this is the case for a few situations (text files), while Spark tends to performance better in most other cases.
S: A bit of advertising, that, much like every paper ever published. Should probably let it be.

3. I also thought that several of the conclusions from the experiments were somewhat misleading. For example, Conclusion 2 mentions that practitioners should choose Arrow-Spark on large datasets, but the performance of the two systems are similar on large datasets. Similarly, Conclusion 5 concludes that Arrow-Spark can leverage projections for parquet files, but so can Spark, and it normally does a better job.
S: Okay, well, I like the conclusions as they are now. Focusing solely on the shortcomings is never good for a paper. This point here is basically an extension on point 2.

What is a ColumnarBatch in Spark?
S: Added clarity at the place where we talk about this.


Evaluation:

What is the specification of the disks used in your experimental setup? Why is it realistic to perform all experiments with data fully cached in DRAM?
S: 1. We primarily use DRAM, not disks. DRAM specs: It is just DRAM, which would be DDR3, unspecified mHz refresh speed. The bottleneck is not on DRAM, so it does not matter much what it is exactly?
S: 2. We already explain why we use DRAM instead of deploying on disks. This is the second reviewer that wants more realistic experiments using disks. We should state more clearly why we went for DRAM tests

In Figure 2, it is hard to see the execution time of Spark and Arrow-Spark since both of them have the same type of circle in the plots.
S: Like everywhere else, it is arrow-spark left, spark right. We already marked the first 3 Arrow-Spark occurrences. It won't get more clear than this.
We could swap this plot for another, but then we lose the emphasis on huge performance variation in Spark, and great performance stability with Arrow-Spark.


Reviewer expertise
------------------
2. I have read some papers in this area

Would the community find this useful if published?
--------------------------------------------------
2. Yes

Correctness
-----------
2. Fixable flaws

Writing
-------
A. Easy to understand

Overall merit
-------------
C. Weak paper, though I will not fight strongly against it


==> tex/__acm_default.tex <==
\section{Submission Instructions}

Submit your PDF file electronically by \textbf{Tuesday, March 2, 2021 (full and short papers) 11:59pm AoE (anywhere on earth)} following the instructions at \url{http://www.systor.org/2021/cfp.html}.

\subsection{Page Limits}
\begin{itemize}
	\item \textbf{Full papers} may include at most 10 pages of content using 10pt font, including everything except references.
	\item \textbf{Short papers} may include at most 5 pages of content using 10pt font, including everything except references.
\end{itemize}

\subsection{Formatting}
\begin{itemize}
	\item
	Please use the ACM latex template for your submission (acmart.cls). This latex file is a simple usage example.
	
	\item
	Categories and subject descriptors are required for the camera-ready version only. You can choose not to include them in your submission. ACM Computing Classification Scheme tool can be found at: https://dl.acm.org/ccs/ccs.cfm
	
	\item
	The review process is \textbf{double-blind}. The "anonymous" parameter keeps authors' name and affiliation hidden, remove it after the review process finishes. Please refer to the sample author block in this document.
	
	\item
	Ensure that the figures and tables are legible.  Please also ensure that you refer to your figures in the main text. Many readers print the papers in gray-scale. Therefore, if you use colors for your figures, ensure that the different colors are distinguishable in gray-scale.
\end{itemize}

\subsection{Citations}

Use a \emph{number} citation format as following~\cite{lamport94,nicepaper,nicepaper2}.

\section{Camera-Ready Submission Instructions}
\begin{itemize}
	
	\item
	Do \textbf{not} include page numbers in the final manuscript.
	
	\item
	Classification and Keywords are only required for the camera-ready version (instructions in tex file).
	
	\item
	Make sure all fonts are embedded in the resulting PDF file.
	
	\item
	Authors will be individually contacted by ACM with instructions on submitting the rights management form. The system will also provide rights management text and a bibliographic strip to appear underneath the copyright notice (ISBN, doi). Authors are responsible for updating their manuscripts with this information.
	
	\item
	The finalized PDF of your paper should be submitted following the instructions at
	\url{http://www.systor.org/2021/cfp.html}.
	
	\item
	The \textbf{deadline} for submitting the final paper and ACM electronic copyright forms is 11:59pm AoE (Anywhere on Earth) May~4, 2021.
\end{itemize}

%Research track	https://systor21.hotcrp.com
%Posters and informal track	https://systor21posters.hotcrp.com
%Highlight track	https://systor21highlight.hotcrp.com


\section*{Acknowledgments}
Acknowledgments are for the camera-ready version only. Please do not include them in your submission.


==> tex/abstract_v0.3.tex <==
Columnar storage formats are increasingly more popular than traditional row-based storage formats in many \acl{ddp} applications, since they have many interesting properties for efficiently reading and storing data.
For certain use-cases, they greatly outperform classical row-storage models.\\
Over the years, researchers created many new columnar storage formats.
Due to the large amount and complexity of columnar storage formats, Apache Arrow was chosen to serve as the de-facto connector between all applications and files producing columnar data.
Apache Arrow is an in-memory columnar data source, supporting all major columnar data types.
There are many secondary storage columnar formats, each with their respective strengths and weaknesses.
However, until recently, there was no common ground for data processing frameworks to
% operate on or
pass around a de-facto in-memory representation.
Apache Arrow recently achieved this standard and is currently integrated with many data processing frameworks.\\
% Recently, Arrow developped a new Dataset API, which allows us to work efficiently with tabular, potentially larger than memory and multi-file datasets, supporting combining different sources.
%% This is most useful for \acl{ddps}s, where data is almost exclusively larger than a single machine's memory capacity.\\
% These features are most useful for \aclp{ddps}, which often work with column-stored data in storage, communication between layers, etc.
The most widely used \acl{ddps} is Apache Spark. Currently, Spark does not support Arrow.
This means Spark is unable to communicate directly with the ever growing group of Arrow-enabled data processing frameworks.
To mitigate this, the Spark community approach is to directly support all columnar storage types.
As a consequence, Spark needs to be updated whenever a new columnar data format emerges.
Additionally, Spark remains unable to communicate directly and efficiently with Arrow-capable data processing frameworks.
In this work, we build a connector between Apache Spark and Apache Arrow, enabling researchers and industry to seamlessly use Spark to access column-stored data from many frameworks and storage engines which use Arrow as mediator.
To benefit the community, we open-source our work and present an in-depth performance evaluation which shows that reading through Apache Arrow is more performant in Spark than using its native Parquet reader.

==> tex/intro_v0.2.tex <==
\section{Introduction}
Distributed data processing frameworks, like Apache Spark~\cite{Spark}, Hadoop~\cite{Hadoop}, or Snowflake~\cite{Snowflake} have become pervasive, being used in most domains of science and technology.
With each advancement in processing units, worldwide processing power significantly increased, and so did data generation.
Statistics~\cite{introstat1} show that this year's (2020) generated data will exceed 59 zettabytes, or approximately $165,730,337$ terabyte every day.
The yearly amount of generated data follows a clear exponential trend where we generate more than twice the amount of data every 3 years, which is expected to continue in the future, as digitization and data processing become ever more important to government, industry and academia. All of this data in itself is not useful.
We use data processing systems to extract useful patterns, statistics, features etc.
We use \aclp{ddps} to process data which is too large or would take too long to be processed by a single machine.

Research, government and industry use \aclp{ddps} for a wide variety of cases, from crime fighting~\cite{Crime1} to disease outbreak management~\cite{DiseaseOutbreak1, DiseaseOutbreak2}, from stock markets~\cite{StockMarket1} to experimental medicine creation~\cite{Medicine1}, all to better understand our perceived world and interact with it more efficiently. There are many different frameworks available to construct and coordinate many different kinds of \aclp{ddps}.
Spark~\cite{Spark} and Hadoop~\cite{Hadoop} perform batch-processing-like computations.
Flink~\cite{Flink} and Storm~\cite{Storm} provide stream processing,
while Kafka~\cite{Kafka} and IBMEventStreams~\cite{IBMEventStreams} provide event streaming.
Highly specialized frameworks also exist, like Ray~\cite{Ray} for distributed machine learning and GraphX~\cite{Graphx} for distributed graph computations.

For years, researchers have worked on ways to optimize \aclp{ddps} or think of new ones, to cope with the large increase and variety in data, and in order to increase processing throughput, reduce cost and improve efficiency.
Even though they were not initially used much in the \acl{ddp} community, column-based storage and communication strategies proved themselves as viable methods to increase data interaction performance in \aclp{ddps}. Well-known columnar data formats include Apache Parquet~\cite{Parquet} and Apache Optimized Row Columnar format (ORC)~\cite{ORC}. The idea of columnar data formats originated from the world of database systems research for improving analytical workloads.~\cite{ColumnOrigin}. Today, many applications interacting with \acl{ddps}s use column-based data in many forms and types. Notable examples include Tensorflow~\cite{Tensorflow} for machine learning,
AWS Data Wrangler~\cite{AWSDataWrangler} for cloud systems,
CuDF~\cite{CuDF} for CUDA-based GPU columnar data processing with Dataframes,
SciDB~\cite{SciDB} for database architectures.

For performance reasons, it is most important to avoid conversion between row- and column based data, as conversion will lead to loss of compression, metadata information, and add a lot of overhead in general.
We must prevent conversion to keep data throughput and efficiency high. More and more applications support data communication through Apache Arrow~\cite{Arrow}.
Arrow is used to read from and write to many different columnar data types, and provides in-memory data representations for them.
Despite these interesting developments, Core Apache Spark~\cite{Spark} lacks the same ability to interact efficiently with Arrow.
Apache Spark is the most widely used \acl{ddp} in industry and many research areas, capable of processing exabyte-scale data in an efficiently distributed manner.
Many frameworks exist to extend Spark, even further increasing Spark's use cases.
Examples include Apache Flink~\cite{Flink}, Storm~\cite{Storm} and Kafka~\cite{Kafka}.

The incompatibility between native Spark and Arrow is an unsolved problem. 
To work on alleviating this problem, in this paper, we aim to answer the following research questions:
\begin{itemize}
    \item[RQ1] How to build a communication bridge between Apache Arrow and Apache Spark, allowing Spark to access data through Arrow?
    \item[RQ2] How does Spark performance compare when using our Arrow support implementation versus using Spark's built-in support? 
    % / What is the relative performance between...
\end{itemize}

We created a connector between Apache Spark and Apache Arrow, and a set of realistic benchmarks, to help us answer these questions, by measuring execution time on large datasets.
\paragraph*{Contributions} The main contributions of this work are:
\begin{itemize}
    \item A proof-of-concept framework to facilitate communication between core Apache Spark and Apache Arrow, and
    \item An in-depth evaluation and comparison of our framework's 
    % reading 
    performance vs default Spark 
    % reading
    performance, in a practical cluster environment setup.
\end{itemize}
